Bayesian analysis of properties of nuclear matter with the FOPI experimental data

Based on the ultra-relativistic quantum molecular dynamics (UrQMD) transport model, combined with experimental data of directed flow, elliptic flow, and nuclear stopping power measured by FOPI in $\rm ^{197}Au+^{197}Au$ collisions at beam energies ($E_{lab}$) of 0.25 and 0.4 GeV/nucleon, the incompressibility of the nuclear equation of state $K_0$, the nucleon effective mass $m^*$, and the in-medium correction factor ($F$, with respect to free-space values) on the nucleon-nucleon elastic cross sections are studied by Bayesian analysis. It is found that both $m^*$ and $F$ can be tightly constrained with the uncertainty $\le$ 15\%, however, $K_0$ cannot be constrained tightly. We deduce $m^*/m_0 = 0.78^{+0.09}_{-0.10}$ and $F = 0.75^{+0.08}_{-0.07}$ with experimental data at $E_{lab}$ = 0.25 GeV/nucleon, and the obtained values increased to $m^*/m_0 = 0.88^{+0.03}_{-0.03}$ and $F = 0.88^{+0.06}_{-0.07}$ at $E_{lab}$ = 0.4 GeV/nucleon. The obtained results are further verified with rapidity-dependent flow data.

==> eos.tex <==
The EoS as functions of density $\rho$ and asymmetry $\delta$ can usually be expressed as:

\begin{equation}
E(\rho, \delta)=E_{0}(\rho)+E_{\mathrm{sym}}(\rho) \delta^{2}+O\left(\delta^{4}\right) \ldots
\end{equation}
where $E_{0}(\rho)$ is the binding energy of isospin symmetric nuclear matter, and $E_{\mathrm{sym}}(\rho)$ is the nuclear symmetry energy. Numerically, $E_{0}(\rho)$ can be expanded around the saturation density $\rho _{0}$ as:

\begin{equation}
E_{0}(\rho)=E_{0}\left(\rho_{0}\right)+\frac{K_{0}}{2!} \chi^{2}+\frac{J_{0}}{3!} \chi^{3}+O\left(\chi^{4}\right),
\end{equation}
with $\chi =(\rho -\rho _{0})/3 \rho _{0}$. $K_{0}=9 \rho_{0}^{2}\left(d^{2} E_{0} / d \rho^{2}\right)_{\rho=\rho_{0}}$ is the incompressibility of isospin symmetric nuclear matter defined at the saturation
density.
